Parallel Algorithms for Finding Large Cliques in Sparse Graphs

We present a parallel k-clique listing algorithm with improved work bounds (for the same depth) in sparse graphs with low degeneracy or arboricity. We achieve this by introducing and analyzing a new pruning criterion for a backtracking search. Our algorithm has better asymptotic performance, especially for larger cliques (when k is not constant), where we avoid the straightforwardly exponential runtime growth with respect to the clique size. In particular, for cliques that are a constant factor smaller than the graph's degeneracy, the work improvement is an exponential factor in the clique size compared to previous results. Moreover, we present a low-depth approximation to the community degeneracy (which can be arbitrarily smaller than the degeneracy). This approximation enables a low depth clique listing algorithm whose runtime is parameterized by the community degeneracy.

==> definitions.tex <==
%\section{Definitions}\label{sec:definitions}
%Here, we provide definitions for all terms that we need to properly derive the work- and depth-complexity of \vref{alg:kcliqueListing}. All relevant symbols are in addition summarized in \vref{tab:commonSymbols}. Some of the notation introduced in \vref{ch:notation} is properly defined here as well.\todo{Notations chapter. Point here}

\begin{table}
	\begin{tabularx}{\textwidth}{rX}
		\toprule
		Symbol &Brief description\\\midrule
		$G = (V,E)$ &Simple graph. Can be directed or undirected.\\
		$E$ &Edges of graph $G=(V,E)$.\\
		$V$ &Vertices of graph $G=(V,E)$.\\
		$N^+(u),\; N^-(u)$ &Out-/In-Neighbors of vertex $u$ in graph $G=(V,E)$.\\
		$N(e) = N(u,v)$ &Neighborhood of an edge (\ie all `the third points' of all triangles associated with it). Default-Definition: $N(u,v) = N^+(u)\cap N^-(v)$.\\
		$G[V']$ &Graph induced on $G = (V,E)$ by vertex set $V'\subseteq V$.\\
		$V[V']$ &Vertices of graph induced on $G=(V,E)$ by vertex set $V'$.\\
		$E[V']$ &Edges of graph induced on $G=(V,E)$ by vertex set $V'$.\\
		$N[V']^+(u),\;N[V']^-(u)$ &Out- (In-)neighbors of vertex $u$ in the graph induced on $G=(V,E)$ by vertex set $V'$.\\
		$N[V'](e) = N[V'](u,v)$ &Neighborhood of edge $e=(u,v)$ in graph induced on $G=(V,E)$ by vertex set $V'$.\\
		$\mathcal{I}(E,c)$ &All edges of $E$ that are important with respect to $c\ge 0$.\\
		$\relevantedge{G}{c}$ &All edges of $E$ that are relevant with respect to $c\ge 0$.\\
		$\relevantpair{V}{c}$ &All pairs of $V\times V$ that are relevant with respect to $c\ge 0$.\\
		$\relevantout{V}{c}$ &All relevant out-vertices in $V$ with respect to $c$.\\
		$\relevantin{V}{c}$ &All relevant in-vertices in $V$ with respect to $c$.\\
		$r(c) = \lfloor(c-2)/2\rfloor$ &Number of recursive calls induced by $c$.\\
		$s$ &Degeneracy (defined later). \\
		$s_c$ &Community Degeneracy (defined later).\\
		$k$ &A constant. Usually the size of the cliques we are searching.\\
		$c$ &A constant. Usually the recursion counter, \ie how many vertices are still missing until we have a $k$-clique.\\
		$I_c$ &Set of candidates. Input to the algorithm at recursion counter $c$.\\
		$T(c, I_c)$ &Cost of recursion at counter $c$ and with input (candidate set) $I_c$.\\
		\bottomrule
	\end{tabularx}
	\caption{The most common symbols used in thesis.}\label{tab:commonSymbols}
\end{table}
